2D Matryoshka Training for Information Retrieval

2D Matryoshka Training is an advanced embedding representation training approach designed to train an encoder model simultaneously across various layer-dimension setups. This method has demonstrated higher effectiveness in Semantic Text Similarity (STS) tasks over traditional training approaches when using sub-layers for embeddings. Despite its success, discrepancies exist between two published implementations, leading to varied comparative results with baseline models. In this reproducibility study, we implement and evaluate both versions of 2D Matryoshka Training on STS tasks and extend our analysis to retrieval tasks. Our findings indicate that while both versions achieve higher effectiveness than traditional Matryoshka training on sub-dimensions, and traditional full-sized model training approaches, they do not outperform models trained separately on specific sub-layer and sub-dimension setups. Moreover, these results generalize well to retrieval tasks, both in supervised (MSMARCO) and zero-shot (BEIR) settings. Further explorations of different loss computations reveals more suitable implementations for retrieval tasks, such as incorporating full-dimension loss and training on a broader range of target dimensions. Conversely, some intuitive approaches, such as fixing document encoders to full model outputs, do not yield improvements. Our reproduction code is available at https://github.com/ielab/2DMSE-Reproduce.

==> sections/tables.tex <==










%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|lll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%	fedweb-13 & query & flan-large & name & 0.1144 & 0.1462 & 0.3527 & 0.1052 & 0.1123 \\
%	fedweb-13 & query & flan-large & name-description & 0.1493 & 0.2027 & 0.4463 & 0.0991 & 0.1303 \\
%	fedweb-13 & query & flan-xl & name & 0.1511 & 0.2054 & 0.4123 & 0.1239 & 0.1374 \\
%	fedweb-13 & query & flan-xl & name-description & 0.1766 & 0.2065 & 0.4252 & 0.1603 & 0.1786 \\
%	fedweb-13 & query & flan-xxl & name & 0.2850 & 0.3217 & 0.5647 & \textbf{0.2939} & 0.2747 \\
%	fedweb-13 & query & flan-xxl & name-description & 0.2938 & \textbf{0.3609} & \textbf{0.5786} & 0.2083 & 0.2797 \\
%	fedweb-13 & query & llama2-13b-chat & name & 0.1015 & 0.1339 & 0.3036 & 0.1045 & 0.1069 \\
%	fedweb-13 & query & llama2-13b-chat & name-description & 0.1059 & 0.1379 & 0.3381 & 0.1153 & 0.0999 \\
%	fedweb-13 & query & llama2-7b-chat & name & 0.0683 & 0.0815 & 0.2626 & 0.0273 & 0.0644 \\
%	fedweb-13 & query & llama2-7b-chat & name-description & 0.1054 & 0.1236 & 0.2748 & 0.0889 & 0.1002 \\
%	fedweb-13 & query & mixtral-13b & name & 0.2605 & 0.3059 & 0.5224 & 0.1897 & 0.2492 \\
%	fedweb-13 & query & mixtral-13b & name-description & \textbf{0.2955} & 0.3451 & 0.5319 & 0.2052 & \textbf{0.2915} \\
%	fedweb-13 & query & solar-11b & name & 0.2636 & 0.3029 & 0.5351 & 0.2713 & 0.2486 \\
%	fedweb-13 & query & solar-11b & name-description & 0.2040 & 0.2667 & 0.5085 & 0.1015 & 0.1838 \\ \midrule
%	
%	fedweb-13 & description & flan-large & name & 0.1620 & 0.1862 & 0.4219 & 0.1514 & 0.1411 \\
%	fedweb-13 & description & flan-large & name-description & 0.2136 & 0.2784 & 0.4879 & 0.1865 & 0.1967 \\
%	fedweb-13 & description & flan-xl & name & 0.1789 & 0.2143 & 0.4384 & 0.1939 & 0.1638 \\
%	fedweb-13 & description & flan-xl & name-description & 0.2089 & 0.2454 & 0.4605 & 0.1916 & 0.2037 \\
%	fedweb-13 & description & flan-xxl & name & 0.2984 & 0.3508 & 0.5725 & 0.3392 & 0.2651 \\
%	fedweb-13 & description & flan-xxl & name-description & 0.3060 & 0.3767 & 0.5814 & 0.2218 & 0.2710 \\
%	fedweb-13 & description & llama2-13b-chat & name & 0.1640 & 0.2140 & 0.4129 & 0.1733 & 0.1564 \\
%	fedweb-13 & description & llama2-13b-chat & name-description & 0.1978 & 0.2590 & 0.4363 & 0.1256 & 0.1612 \\
%	fedweb-13 & description & llama2-7b-chat & name & 0.1156 & 0.1467 & 0.3599 & 0.0780 & 0.1045 \\
%	fedweb-13 & description & llama2-7b-chat & name-description & 0.1652 & 0.1973 & 0.3810 & 0.1876 & 0.1607 \\
%	fedweb-13 & description & mixtral-13b & name & 0.2802 & 0.3246 & 0.5562 & 0.2392 & 0.2726 \\
%	fedweb-13 & description & mixtral-13b & name-description & 0.3333 & \textbf{0.3978} & 0.5830 & 0.3109 & 0.3037 \\
%	fedweb-13 & description & solar-11b & name & \textbf{0.3573} & 0.3944 & \textbf{0.5982} & \textbf{0.3809} & \textbf{0.3398} \\
%	fedweb-13 & description & solar-11b & name-description & 0.2917 & 0.3541 & 0.5674 & 0.2692 & 0.2699 \\
%	
%	
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:n}
%\end{table*}
%
%
%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|llll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&top-n&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%
%fedweb-13 &query & flan-large & example-snippet & 1 & 0.1485 & 0.1918 & 0.4076 & 0.0973 & 0.1527 \\
%fedweb-13 &query & flan-large & example-snippet & 2 & 0.1718 & 0.2106 & 0.4324 & 0.1337 & 0.1545 \\
%fedweb-13 &query & flan-large & example-snippet & 3 & 0.1619 & 0.2079 & 0.4377 & 0.1048 & 0.1464 \\
%fedweb-13 &query & flan-large & example-snippet & 5 & 0.1918 & 0.2367 & 0.4558 & 0.1877 & 0.1701 \\ \midrule
%fedweb-13 &query & flan-xl & example-snippet & 1 & 0.1310 & 0.1605 & 0.3655 & 0.0923 & 0.1280 \\
%fedweb-13 &query & flan-xl & example-snippet & 2 & 0.1369 & 0.1774 & 0.3957 & 0.0844 & 0.1264 \\
%fedweb-13 &query & flan-xl & example-snippet & 3 & 0.1509 & 0.1853 & 0.4131 & 0.1044 & 0.1258 \\
%fedweb-13 &query & flan-xl & example-snippet & 5 & 0.1706 & 0.1982 & 0.4239 & 0.1487 & 0.1498 \\ \midrule
%fedweb-13 & query & flan-xxl & example-snippet & 1 & 0.2179 & 0.2673 & 0.4779 & 0.1404 & 0.2067 \\
%fedweb-13 & query & flan-xxl & example-snippet & 2 & 0.2295 & 0.2884 & 0.5107 & 0.1632 & 0.2156 \\
%fedweb-13 & query & flan-xxl & example-snippet & 3 & 0.2412 & 0.2801 & 0.5126 & 0.1761 & 0.2395 \\
%fedweb-13 & query & flan-xxl & example-snippet & 5 & 0.2382 & 0.2950 & \textbf{0.5155} & 0.1579 & 0.2181 \\ \midrule
%fedweb-13 & query & mixtral-13b & example-snippet & 1 & 0.2375 & 0.2849 & 0.4699 & 0.1633 & \textbf{0.2418} \\
%fedweb-13 & query & mixtral-13b & example-snippet & 2 & \textbf{0.2464} & 0.2861 & 0.4770 & 0.2224 & 0.2102 \\
%fedweb-13 & query & mixtral-13b & example-snippet & 3 & 0.2319 & \textbf{0.2966} & 0.4835 & \textbf{0.2406} & 0.1909 \\
%fedweb-13 & query & mixtral-13b & example-snippet & 5 & 0.2310 & 0.2947 & 0.4993 & 0.1946 & 0.2165 \\ \midrule
%fedweb-13 & query & solar-11b & example-snippet & 1 & 0.2186 & 0.2757 & 0.4850 & 0.1399 & 0.1848 \\
%fedweb-13 & query & solar-11b & example-snippet & 2 & 0.1944 & 0.2479 & 0.4634 & 0.0955 & 0.1784 \\
%fedweb-13 & query & solar-11b & example-snippet & 3 & 0.1883 & 0.2509 & 0.4829 & 0.1914 & 0.1609 \\
%fedweb-13 & query & solar-11b & example-snippet & 5 & 0.1356 & 0.2099 & 0.4595 & 0.1058 & 0.1176 \\ \midrule
%fedweb-13 &description & flan-large & example-snippet & 1 & 0.1457 & 0.1898 & 0.3877 & 0.1323 & 0.1355 \\
%fedweb-13 &description & flan-large & example-snippet & 2 & 0.1871 & 0.2337 & 0.4287 & 0.2331 & 0.1718 \\
%fedweb-13 &description & flan-large & example-snippet & 3 & 0.2024 & 0.2388 & 0.4481 & 0.2068 & 0.1859 \\
%fedweb-13 &description & flan-large & example-snippet & 5 & 0.2070 & 0.2477 & 0.4529 & 0.2540 & 0.1745 \\ \midrule
%fedweb-13 &description & flan-xl & example-snippet & 1 & 0.1701 & 0.2122 & 0.4089 & 0.0997 & 0.1735 \\
%fedweb-13 &description & flan-xl & example-snippet & 2 & 0.1840 & 0.2283 & 0.4442 & 0.1727 & 0.1771 \\
%fedweb-13 &description & flan-xl & example-snippet & 3 & 0.1867 & 0.2236 & 0.4540 & 0.1484 & 0.1788 \\
%fedweb-13 &description & flan-xl & example-snippet & 5 & 0.1788 & 0.2219 & 0.4471 & 0.1302 & 0.1607 \\\midrule
%fedweb-13 & description & flan-xxl & example-snippet & 1 & 0.2795 & 0.3427 & 0.5388 & 0.2201 & 0.2470 \\
%fedweb-13 & description & flan-xxl & example-snippet & 2 & 0.3183 & 0.3810 & 0.5791 & 0.2804 & 0.2863 \\
%fedweb-13 & description & flan-xxl & example-snippet & 3 & \textbf{0.3378} & 0.3844 & \textbf{0.5948} & 0.3102 & 0.3163 \\ 
%fedweb-13 & description & flan-xxl & example-snippet & 5 & 0.3167 & 0.3883 & 0.5835 & 0.2671 & 0.2885 \\ \midrule
%fedweb-13 & description & mixtral-13b & example-snippet & 1 & 0.3024 & 0.3476 & 0.4864 & 0.2840 & 0.2973 \\
%fedweb-13 & description & mixtral-13b & example-snippet & 2 & 0.2824 & 0.3121 & 0.4665 & 0.2547 & 0.2989 \\
%fedweb-13 & description & mixtral-13b & example-snippet & 3 & 0.3234 & 0.3535 & 0.4995 & \textbf{0.3593} & 0.2929 \\
%fedweb-13 & description & mixtral-13b & example-snippet & 5 & 0.3363 & 0.3825 & 0.5279 & 0.3575 & 0.3076 \\ \midrule
%fedweb-13 & description & solar-11b & example-snippet & 1 & 0.3346 & \textbf{0.3905} & 0.5634 & 0.3362 & \textbf{0.3267} \\
%fedweb-13 & description & solar-11b & example-snippet & 2 & 0.3221 & 0.3594 & 0.5411 & 0.3532 & 0.3104 \\
%fedweb-13 & description & solar-11b & example-snippet & 3 & 0.3106 & 0.3522 & 0.5544 & 0.2724 & 0.3068 \\
%fedweb-13 & description & solar-11b & example-snippet & 5 & 0.2417 & 0.3135 & 0.5325 & 0.2091 & 0.2160 \\
%		
%		
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:3}
%\end{table*}
%
%
%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|lll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%fedweb-14 & query & flan-large & name & 0.1249 & 0.1544 & 0.3450 & 0.0933 & 0.1111 \\
%fedweb-14 & query & flan-large & name-description & 0.2073 & 0.2461 & 0.4818 & 0.1210 & 0.1952 \\
%fedweb-14 & query & flan-xl & name & 0.1484 & 0.1845 & 0.3799 & 0.1097 & 0.1377 \\
%fedweb-14 & query & flan-xl & name-description & 0.1480 & 0.1833 & 0.3882 & 0.1097 & 0.1368 \\
%fedweb-14 & query & flan-xxl & name & 0.2568 & 0.2984 & 0.5428 & 0.2508 & 0.2307 \\
%fedweb-14 & query & flan-xxl & name-description & 0.3231 & 0.3882 & 0.5856 & 0.2087 & 0.3071 \\
%fedweb-14 & query & llama2-13b-chat & name & 0.0977 & 0.1184 & 0.3370 & 0.1047 & 0.0856 \\
%fedweb-14 & query & llama2-13b-chat & name-description & 0.0951 & 0.1226 & 0.3373 & 0.0706 & 0.0988 \\
%fedweb-14 & query & llama2-7b-chat & name & 0.0529 & 0.0717 & 0.2500 & 0.0232 & 0.0441 \\
%fedweb-14 & query & llama2-7b-chat & name-description & 0.0698 & 0.0934 & 0.2435 & 0.0510 & 0.0688 \\
%fedweb-14 & query & mixtral-13b & name & 0.2870 & 0.3431 & 0.5614 & 0.2896 & 0.2572 \\
%fedweb-14 & query & mixtral-13b & name-description & 0.3025 & 0.3555 & 0.5537 & 0.2267 & 0.2642 \\
%fedweb-14 & query & solar-11b & name & \textbf{0.4093} & \textbf{0.4227} & \textbf{0.6115} & \textbf{0.3931} & \textbf{0.3926} \\
%fedweb-14 & query & solar-11b & name-description & 0.2497 & 0.3163 & 0.5406 & 0.0783 & 0.2280 \\ \midrule
%
%fedweb-14 & description & flan-large & name & 0.1810 & 0.1999 & 0.4139 & 0.1924 & 0.1692 \\
%fedweb-14 & description & flan-large & name-description & 0.2581 & 0.2906 & 0.5062 & 0.1881 & 0.2699 \\
%fedweb-14 & description & flan-xl & name & 0.1801 & 0.2092 & 0.4087 & 0.1717 & 0.1866 \\
%fedweb-14 & description & flan-xl & name-description & 0.1996 & 0.2350 & 0.4303 & 0.1609 & 0.2024 \\
%fedweb-14 & description & flan-xxl & name & 0.2705 & 0.3213 & 0.5528 & 0.3408 & 0.2410 \\
%fedweb-14 & description & flan-xxl & name-description & 0.3289 & 0.3898 & 0.5917 & 0.3128 & 0.3022 \\
%fedweb-14 & description & llama2-13b-chat & name & 0.1599 & 0.1945 & 0.4008 & 0.1987 & 0.1401 \\
%fedweb-14 & description & llama2-13b-chat & name-description & 0.1381 & 0.1942 & 0.3965 & 0.0835 & 0.1261 \\
%fedweb-14 & description & llama2-7b-chat & name & 0.0606 & 0.0976 & 0.3132 & 0.0355 & 0.0594 \\
%fedweb-14 & description & llama2-7b-chat & name-description & 0.1067 & 0.1209 & 0.3184 & 0.0874 & 0.1040 \\
%fedweb-14 & description & mixtral-13b & name & 0.2927 & 0.3558 & 0.5680 & 0.2980 & 0.2653 \\
%fedweb-14 & description & mixtral-13b & name-description & 0.3163 & 0.3762 & 0.5797 & 0.2855 & 0.2768 \\
%fedweb-14 & description & solar-11b & name & \textbf{0.4351} & \textbf{0.4509} & \textbf{0.6362} & \textbf{0.3803} & \textbf{0.4363} \\
%fedweb-14 & description & solar-11b & name-description & 0.3205 & 0.3730 & 0.5764 & 0.1999 & 0.2859 \\
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:2}
%\end{table*}
%
%
%
%
%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|llll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&top-n&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%fedweb-14 & query & flan-xxl & example-snippet & 1 & 0.2431 & 0.2942 & 0.5022 & 0.1293 & 0.2402 \\
%fedweb-14 & query & flan-xxl & example-snippet & 2 & 0.2559 & 0.3058 & 0.5213 & 0.1904 & 0.2372 \\
%fedweb-14 & query & flan-xxl & example-snippet & 3 & 0.2917 & 0.3278 & 0.5412 & 0.2638 & 0.2418 \\
%fedweb-14 & query & flan-xxl & example-snippet & 5 & 0.2621 & 0.3258 & 0.5358 & 0.2128 & 0.2220 \\ \midrule
%fedweb-14 & query & mixtral-13b & example-snippet & 1 & 0.1903 & 0.2426 & 0.4443 & 0.0974 & 0.1771 \\
%fedweb-14 & query & mixtral-13b & example-snippet & 2 & 0.2057 & 0.2665 & 0.4643 & 0.1232 & 0.1906 \\
%fedweb-14 & query & mixtral-13b & example-snippet & 3 & 0.1929 & 0.2508 & 0.4704 & 0.1415 & 0.1675 \\
%fedweb-14 & query & mixtral-13b & example-snippet & 5 & 0.1792 & 0.2582 & 0.4784 & 0.1390 & 0.1526 \\ \midrule
%fedweb-14 & query & solar-11b & example-snippet & 1 & \textbf{0.3095} & \textbf{0.3505} & \textbf{0.5417} & \textbf{0.3061} & \textbf{0.2897} \\
%fedweb-14 & query & solar-11b & example-snippet & 2 & 0.2051 & 0.2581 & 0.4769 & 0.1746 & 0.1680 \\
%fedweb-14 & query & solar-11b & example-snippet & 3 & 0.1739 & 0.2346 & 0.4774 & 0.1204 & 0.1670 \\
%fedweb-14 & query & solar-11b & example-snippet & 5 & 0.1581 & 0.2133 & 0.4617 & 0.1045 & 0.1398 \\ \midrule
%
%fedweb-14 & description & flan-xxl & example-snippet & 1 & 0.3066 & 0.3565 & 0.5468 & \textbf{0.3136} & 0.2777 \\
%fedweb-14 & description & flan-xxl & example-snippet & 2 & \textbf{0.3128} & \textbf{0.3647} & 0.5583 & 0.1998 & 0.2889 \\
%fedweb-14 & description & flan-xxl & example-snippet & 3 & 0.2958 & 0.3594 & \textbf{0.5628} & 0.2511 & 0.2753 \\
%fedweb-14 & description & flan-xxl & example-snippet & 5 & 0.2855 & 0.3472 & 0.5564 & 0.2383 & 0.2645 \\ \midrule
%fedweb-14 & description & mixtral-13b & example-snippet & 1 & 0.2532 & 0.2912 & 0.4652 & 0.1880 & 0.2114 \\
%fedweb-14 & description & mixtral-13b & example-snippet & 2 & 0.2823 & 0.3185 & 0.4774 & 0.2066 & 0.2792 \\
%fedweb-14 & description & mixtral-13b & example-snippet & 3 & 0.2784 & 0.3187 & 0.4879 & 0.1793 & 0.2646 \\
%fedweb-14 & description & mixtral-13b & example-snippet & 5 & 0.2885 & 0.3486 & 0.5168 & 0.2616 & 0.2675 \\ \midrule
%fedweb-14 & description & solar-11b & example-snippet & 1 & 0.2999 & 0.3490 & 0.5413 & 0.3110 & \textbf{0.2917} \\
%fedweb-14 & description & solar-11b & example-snippet & 2 & 0.2465 & 0.3001 & 0.5159 & 0.2335 & 0.2322 \\
%fedweb-14 & description & solar-11b & example-snippet & 3 & 0.2145 & 0.2907 & 0.5118 & 0.1757 & 0.1988 \\
%fedweb-14 & description & solar-11b & example-snippet & 5 & 0.1849 & 0.2628 & 0.4966 & 0.1159 & 0.1549 \\
%		
%		
%		
%		
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:4}
%\end{table*}
%
%
%\begin{table*}
%	\centering
%	
%	\begin{tabular}{l|lll|lllll}
%		\toprule
%		
%		Dataset&$R(query)$&LLM&$R(Resource)$&ndcg10&ndcg20&ndcg100& nP1&nP5 \\ \midrule
%		fedweb-13 &/&all-best&/&&0.2990&/&0.1600&0.2100\\
%		fedweb-13 &/&no-info-used&/&&0.1850&/&0.0700&0.1000\\
%		fedweb-13 & query & flan-large & name & 0.7461 & 0.7764 & 0.8515 & 0.6945 & 0.7539 \\
%		fedweb-13 & query & flan-large & name-description & 0.7349 & 0.7789 & 0.8496 & 0.6914 & 0.7499 \\
%		fedweb-13 & query & flan-xl & name & \textbf{0.7557} & \textbf{0.7897} & \textbf{0.8574} & 0.6929 & \textbf{0.7752} \\
%		fedweb-13 & query & flan-xl & name-description & 0.7533 & 0.7830 & 0.8554 & 0.6929 & 0.7676 \\
%		fedweb-13 & query & llama2-7b-chat & name & 0.7302 & 0.7729 & 0.8494 & \textbf{0.7612} & 0.7680 \\
%		fedweb-13 & query & llama2-7b-chat & name-description & 0.7428 & 0.7572 & 0.8397 & 0.6686 & 0.7470 \\ \midrule
%		fedweb-13 & description & flan-large & name & 0.7501 & 0.7932 & 0.8593 & 0.6929 & 0.7714 \\
%		fedweb-13 & description & flan-large & name-description & 0.7459 & 0.7910 & 0.8553 & \textbf{0.7085} & 0.7547 \\
%		fedweb-13 & description & flan-xl & name & \textbf{0.7556} & \textbf{0.7988} & \textbf{0.8622} & 0.6950 & \textbf{0.7857} \\
%		fedweb-13 & description & flan-xl & name-description & 0.7459 & 0.7859 & 0.8540 & 0.6844 & 0.7623 \\
%		fedweb-13 & description & llama2-7b-chat & name & 0.7090 & 0.7613 & 0.8349 & 0.6781 & 0.7562 \\ \midrule \midrule
%		
%		
%		fedweb-14 &/&all-best&/&0.6010&0.7000&/&0.5250&0.5790\\
%		fedweb-14 &/&no-learning-on-human&/&0.4260&0.5170&/&0.2710&0.4040\\
%		fedweb-14 & query & flan-large & name & 0.6265 & 0.6927 & 0.7768 & 0.3060 & 0.6970 \\
%		fedweb-14 & query & flan-large & name-description & 0.6418 & 0.6995 & 0.7809 & 0.3060 & 0.7210 \\
%		fedweb-14 & query & flan-xl & name & 0.6582 & 0.7088 & 0.7855 & 0.3060 & 0.6854 \\
%		fedweb-14 & query & flan-xl & name-description & \textbf{0.6639} & 0.7077 & \textbf{0.7877} & 0.3060 & \textbf{0.7299} \\
%		fedweb-14 & query & llama2-7b-chat & name & 0.5476 & 0.6228 & 0.7111 & \textbf{0.3483} & 0.4816 \\
%		fedweb-14 & query & llama2-7b-chat & name-description & 0.6568 & \textbf{0.7106} & 0.7811 & 0.3060 & 0.6975 \\ \midrule
%		fedweb-14 & description & flan-large & name & 0.6608 & \textbf{0.7158} & 0.7897 & \textbf{0.3230} & \textbf{0.7516} \\
%		fedweb-14 & description & flan-large & name-description & \textbf{0.6736} & 0.7152 & \textbf{0.7902} & 0.3060 & 0.7407 \\
%		fedweb-14 & description & flan-xl & name & 0.6557 & 0.7052 & 0.7833 & 0.3060 & 0.7008 \\
%		fedweb-14 & description & flan-xl & name-description & 0.6608 & 0.6999 & 0.7849 & 0.3060 & 0.7054 \\
%		fedweb-14 & description & llama2-7b-chat & name & 0.6499 & 0.6984 & 0.7683 & 0.3060 & 0.6913 \\
%		fedweb-14 & description & llama2-7b-chat & name-description & 0.6232 & 0.6923 & 0.7577 & 0.3060 & 0.6413 \\
%		
%		\bottomrule
%	\end{tabular}
%	\caption{}
%	\label{table:2}
%\end{table*}
%


==> table_prompt_labeling.tex <==
%\begin{tabular}{p{2pt}|M{455pt}}
%	\toprule
%	& \textnormal{Prompt} \\
%	\hline
%	\rotatebox[origin=c]{90}{System Prompt} &  Given a query and a web snippet, you must provide a score on an integer scale of 0 to 4 with the following meanings:\linebreak 4 = navigational, this page represents a home page of an entity directly named by the query; the user may be searching for this specific page or site.\linebreak 3 = top relevance, this page or site is dedicated to the topic; authoritative and comprehensive, it is worthy of being a top result in a web search engine.\linebreak  2 = highly relevant, the content of this page provides substantial information on the topic.\linebreak 2 = highly relevant, the content of this page provides substantial information on the topic.\linebreak 1 = minimal relevance, the content of this page provides some information on the topic, which may be minimal; the relevant information must be on that page, not just promising-looking anchor text pointing to a possibly useful page.\linebreak 0 = not relevant, the content of this page does not provide useful information on the topic, but may provide useful information on other topics, including other interpretations of the same query. \\ \midrule
%	
%	\rotatebox[origin=c]{90}{{\centering User Prompt}} & Assume that you are writing a report on the subject of the topic. mark the web snippet according to the previous scale description.\linebreak Query:\linebreak A person has typed \{query\} into a search engine.\linebreak Result:\linebreak Consider the following web snippet:\linebreak —BEGIN WEB Snippet CONTENT—\linebreak \{snippet\}\linebreak —END WEB Snippet CONTENT—\linebreak Instructions:\linebreak Split this problem into steps:\linebreak Consider the underlying intent of the search.\linebreak Measure how well the content matches a likely intent of the query (M)\linebreak Measure how trustworthy the web page is (T).\linebreak Consider the aspects above and the relative importance of each, and decide on a final score (O).\linebreak Produce a JSON of scores without providing any reasoning. Example:\{"M": 2, "T": 1,"O": 1\}\linebreak Results:\\
%	\bottomrule
%\end{tabular}


==> tables/table_retrieval_base.tex <==
\begin{table}[ht]
	\centering
	\tiny
	\label{tab:retrieval_main}
	\caption{Average Result of Retrieval datasets. Spearman's Correlation is used as the evaluation metrics.}

		\begin{tabular}{l|l|cccccccc}
			\toprule
			& \textbf{Method} & \multicolumn{8}{c|}{V1}\\ 
			\midrule
			\textbf{L} & & \textbf{8} & \textbf{16} & \textbf{32} & \textbf{64} & \textbf{128} & \textbf{256} & \textbf{512} & \textbf{768} \\ 
			\midrule
			
			
			\bottomrule
		\end{tabular}
	
\end{table}

==> tables/table_sts_base.tex <==
\begin{table}[ht]
	\centering
	\tiny
	\label{tab:sts_main}
	\caption{Average Result of STS datasets. Spearman's Correlation is used as the evaluation metrics.}
	\resizebox{\textwidth}{!}{
	\begin{tabular}{l|l|cccccccc|cccccccc}
		\toprule
		\multirow{2}{*}{\rotatebox{90}{Layer}} & \textbf{Method} & \multicolumn{8}{c|}{V1} & \multicolumn{8}{c}{V2} \\ 
		\cmidrule{2-18}
		&	 & \textbf{8} & \textbf{16} & \textbf{32} & \textbf{64} & \textbf{128} & \textbf{256} & \textbf{512} & \textbf{768} & \textbf{8} & \textbf{16} & \textbf{32} & \textbf{64} & \textbf{128} & \textbf{256} & \textbf{512} & \textbf{768} \\ 
		\midrule
	
	\multirow{4}{*}{\rotatebox{90}{2}} 
	& BERT    & 0.444 & 0.522 & 0.578 & 0.607 & 0.624 & 0.634 & 0.574 & 0.589 & 0.253 & 0.297 & 0.313 & 0.335 & 0.339 & 0.335 & 0.335 & 0.337 \\
	& BERT-S       & 0.547 & \textbf{0.630} & \textbf{0.676} & \textbf{0.699} & \textbf{0.715} & \textbf{0.724} & \textbf{0.728} & \textbf{0.730} & \textbf{0.576} & \textbf{0.633} & \textbf{0.669} & \textbf{0.688} & \textbf{0.695} & \textbf{0.700} & \textbf{0.708} & \textbf{0.708} \\
	& MSE         & 0.441 & 0.520 & 0.575 & 0.608 & 0.627 & 0.635 & 0.576 & 0.590 & 0.264 & 0.322 & 0.332 & 0.351 & 0.357 & 0.354 & 0.351 & 0.352 \\
	& 2DMSE       & \textbf{0.559} & 0.621 & 0.656 & 0.674 & 0.681 & 0.684 & 0.675 & 0.680 & 0.504 & 0.603 & 0.644 & 0.669 & 0.675 & 0.684 & 0.684 & 0.685 \\
	\midrule
	
	\multirow{4}{*}{\rotatebox{90}{4}} 
	& BERT    & 0.428 & 0.488 & 0.536 & 0.562 & 0.582 & 0.591 & 0.552 & 0.563 & 0.464 & 0.535 & 0.573 & 0.584 & 0.593 & 0.595 & 0.589 & 0.594 \\
	& BERT-S       & 0.570 & \textbf{0.642} & \textbf{0.699} & \textbf{0.723} & \textbf{0.738} & \textbf{0.744} & \textbf{0.749} & \textbf{0.751} & \textbf{0.620} & \textbf{0.671} & \textbf{0.702} & \textbf{0.722} & \textbf{0.730} & \textbf{0.735} & \textbf{0.738} & \textbf{0.737} \\
	& MSE         & 0.438 & 0.497 & 0.535 & 0.561 & 0.583 & 0.593 & 0.557 & 0.568 & 0.479 & 0.546 & 0.579 & 0.591 & 0.599 & 0.602 & 0.602 & 0.606 \\
	& 2DMSE       & \textbf{0.571} & 0.627 & 0.660 & 0.674 & 0.681 & 0.683 & 0.662 & 0.669 & 0.542 & 0.636 & 0.682 & 0.707 & 0.716 & 0.721 & 0.722 & 0.723 \\
	\midrule
	
	\multirow{4}{*}{\rotatebox{90}{6}} 
	& BERT    & 0.463 & 0.502 & 0.529 & 0.555 & 0.565 & 0.563 & 0.566 & 0.572 & 0.433 & 0.483 & 0.518 & 0.536 & 0.543 & 0.545 & 0.543 & 0.547 \\
	& BERT-S       & 0.578 & \textbf{0.654} & \textbf{0.712} & \textbf{0.743} & \textbf{0.756} & \textbf{0.761} & \textbf{0.765} & \textbf{0.767} & \textbf{0.585} & \textbf{0.670} & \textbf{0.723} & \textbf{0.750} & \textbf{0.757} & \textbf{0.761} & \textbf{0.761} & \textbf{0.763} \\
	& MSE         & 0.464 & 0.513 & 0.533 & 0.557 & 0.572 & 0.569 & 0.577 & 0.583 & 0.428 & 0.483 & 0.514 & 0.539 & 0.544 & 0.549 & 0.550 & 0.554 \\
	& 2DMSE       & \textbf{0.588} & 0.637 & 0.671 & 0.687 & 0.690 & 0.690 & 0.673 & 0.681 & 0.561 & 0.646 & 0.699 & 0.729 & 0.736 & 0.732 & 0.737 & 0.737 \\
	\midrule
	
	\multirow{4}{*}{\rotatebox{90}{8}} 
	& BERT    & 0.475 & 0.522 & 0.549 & 0.581 & 0.592 & 0.591 & 0.593 & 0.600 & 0.364 & 0.406 & 0.424 & 0.455 & 0.460 & 0.457 & 0.464 & 0.466 \\
	& BERT-S       & \textbf{0.612} & \textbf{0.677} & \textbf{0.736} & \textbf{0.763} & \textbf{0.778} & \textbf{0.782} & \textbf{0.786} & \textbf{0.788} & \textbf{0.620} & \textbf{0.690} & \textbf{0.738} & \textbf{0.766} & \textbf{0.776} & \textbf{0.782} & \textbf{0.787} & \textbf{0.790} \\
	& MSE         & 0.486 & 0.542 & 0.556 & 0.590 & 0.608 & 0.610 & 0.622 & 0.626 & 0.417 & 0.452 & 0.470 & 0.505 & 0.512 & 0.508 & 0.515 & 0.516 \\
	& 2DMSE       & 0.600 & 0.647 & 0.683 & 0.703 & 0.709 & 0.710 & 0.698 & 0.702 & 0.587 & 0.658 & 0.709 & 0.743 & 0.753 & 0.751 & 0.756 & 0.757 \\
	\midrule
	
	\multirow{4}{*}{\rotatebox{90}{10}} 
	& BERT   & 0.572 & 0.631 & 0.672 & 0.693 & 0.702 & 0.708 & 0.711 & 0.717 & 0.498 & 0.569 & 0.597 & 0.621 & 0.624 & 0.632 & 0.619 & 0.624 \\
	& BERT-S     & 0.619 & \textbf{0.692} & \textbf{0.748} & \textbf{0.772} & \textbf{0.785} & \textbf{0.793} & \textbf{0.796} & \textbf{0.798} & \textbf{0.636} & \textbf{0.701} & \textbf{0.750} & \textbf{0.777} & \textbf{0.788} & \textbf{0.797} & \textbf{0.800} & \textbf{0.804} \\
	& MSE        & 0.603 & 0.659 & 0.689 & 0.717 & 0.729 & 0.735 & 0.744 & 0.747 & 0.530 & 0.585 & 0.616 & 0.641 & 0.649 & 0.656 & 0.648 & 0.653 \\
	& 2DMSE      & \textbf{0.639} & 0.686 & 0.721 & 0.736 & 0.745 & 0.750 & 0.744 & 0.752 & 0.577 & 0.649 & 0.709 & 0.744 & 0.754 & 0.753 & 0.745 & 0.749 \\
	\midrule
	
	\multirow{4}{*}{\rotatebox{90}{12}} 
	& BERT   & 0.644 & 0.718 & 0.762 & 0.786 & \textbf{0.802} & \textbf{0.810} & \textbf{0.813} & \textbf{0.816} & \textbf{0.646} & \textbf{0.720} & 0.763 & 0.791 & 0.804 & 0.811 & \textbf{0.813} & \textbf{0.816} \\
	& BERT-S     & 0.644 & 0.718 & 0.762 & 0.786 & \textbf{0.802} & \textbf{0.810} & \textbf{0.813} & \textbf{0.816} & \textbf{0.646} & \textbf{0.720} & 0.763 & 0.791 & 0.804 & 0.811 & \textbf{0.813} & \textbf{0.816} \\
	& MSE        & \textbf{0.694} & \textbf{0.753} & \textbf{0.778} & \textbf{0.790} & 0.798 & 0.802 & 0.808 & 0.809 & 0.613 & 0.704 & \textbf{0.764} & \textbf{0.796} & \textbf{0.810} & \textbf{0.813} & \textbf{0.813} & \textbf{0.816} \\
	& 2DMSE     & 0.680 & 0.735 & 0.765 & 0.779 & 0.787 & 0.791 & 0.794 & 0.795 & 0.614 & 0.701 & 0.761 & 0.795 & 0.808 & 0.812 & 0.811 & 0.815 \\
	\bottomrule
	\end{tabular}
}
\end{table}
